A learning-based multiscale method and its application to inelastic impact problems

The macroscopic properties of materials that we observe and exploit in engineering application result from complex interactions between physics at multiple length and time scales: electronic, atomistic, defects, domains etc. Multiscale modeling seeks to understand these interactions by exploiting the inherent hierarchy where the behavior at a coarser scale regulates and averages the behavior at a finer scale. This requires the repeated solution of computationally expensive finer-scale models, and often a priori knowledge of those aspects of the finer-scale behavior that affect the coarser scale (order parameters, state variables, descriptors, etc.). We address this challenge in a two-scale setting where we learn the fine-scale behavior from off-line calculations and then use the learnt behavior directly in coarse scale calculations. The approach draws from recent successes of deep neural networks, in combination with ideas from model reduction. The approach builds on the recent success of deep neural networks by combining their approximation power in high dimensions with ideas from model reduction. It results in a neural network approximation that has high fidelity, is computationally inexpensive, is independent of the need for a priori knowledge, and can be used directly in the coarse scale calculations. We demonstrate the approach on problems involving the impact of magnesium, a promising light-weight structural and protective material.

==> macros.tex <==
\newcommand{\real}{\mathbb{R}}
\newcommand{\rE}{\mathbb{E}}
\newcommand{\rP}{\mathbb{P}}
\newcommand{\L}{\mathcal{L}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bF}{\boldsymbol{F}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\s}{\boldsymbol{s}}
\newcommand{\m}{\boldsymbol{m}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\Q}{\boldsymbol{Q}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\ep}{\epsilon}
\newcommand{\dep}{\dot{\epsilon}}
\newcommand{\bep}{\boldsymbol{\epsilon}}
\newcommand{\dbep}{\boldsymbol{\dot{\epsilon}}}
\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\ga}{\gamma}
\newcommand{\bga}{\boldsymbol{\gamma}}
\newcommand{\dga}{\dot{\gamma}}
\newcommand{\blm}{\boldsymbol{\lambda}}
\newcommand{\dblm}{\boldsymbol{\dot{\lambda}}}
\newcommand{\lm}{\lambda}
\newcommand{\dlm}{\dot{\lambda}}
\newcommand{\md}{\boldsymbol{\sigma}_{M}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\siginf}{{\sigma}_{\alpha}^{\infty}}
\newcommand{\bsig}{\boldsymbol{\sigma}}
\newcommand{\strain}{\varepsilon} 












==> old/Sections/1-Intro.tex <==
\section{Introduction} 
Crystal plasticity has been a phenomenal success in modelling the non-linear, path-dependent behavior of crystalline solids (\cite{Asaro1983CrystalPlasticity}). By modelling the plastic deformation as simple shears along the material slip systems, the crystal plasticity formulation is capable of accurately predicting the finite strain response and the associated texture evolution for a variety of metals with distinct lattice structures. Indeed, the formulation has been applied and experimentally verified for quantifying the single as well as poly-crystalline response of metals including Aluminum (FCC) (\cite{Wu1998CrystalSheets,Lu2011CrystalCrystal,Groh2009MultiscaleCrystal}),  Copper(\cite{Kysar2001ContinuumBackground,Casals2007CrystalCrystals}), Iron (\cite{Koester2012AtomisticallyIron,Barton2013AIron}), Tantalum (BCC)  (\cite{Lim2014Grain-scaleOligocrystals, Kothari1998Elasto-viscoplasticTantalum}), Magnesium (\cite{Chang2015AMagnesium, Zhang2012PhenomenologicalMagnesium}), and Titanium (HCP)  (\cite{Salem2005StrainModeling, Venkatramani2007AAlloys}). Recent studies have further extended the framework to model other inelastic behavior of metals (e.g. twinning\cite{Kalidindi1998IncorporationModels}), as well as to predict the anisotropic plastic behavior of fibre-reinforcement composites (\cite{Liu2019DeepPunch, Tan2020AComposites}). 

Despite its great success in quantifying the detailed micro-mechanical evolution of materials, directly resolving the crystal plasticity model in large-scale, macroscopic simulation with finite deformation has been prohibitive due to the limitation of computational power. For instance, one representative volume element (RVE) calculation of polycrystalline Magnesium requires approximately 10 hours to finish using the modern high performance computing cluster, while typical sequential multi-scale simulation techniques (e.g., $\text{FE}^2$) \cite{Feyel2003AContinua} requires hundreds and thousands of these realisations to analyze one practical engineering problem such as structural impact. On the other hand, classical solid mechanics addresses this issue by considering phenomenological constitutive laws (e.g., Johnson Cook, Hill) \cite{Hill1979TheoreticalAggregates, Johnson2018ATEMPERATURES} where empirical-based relations are postulated for the macroscopic material behavior. However, new models/frameworks have to be re-developed for different materials and their fidelity heavily depends on the a priori assumption of the phenomenological relation. Furthermore, such approaches lack the ability to incorporate sub-scale mechanics and physics which are crucial for complex/novel material and structural systems.  

Recent advance in data-driven computational methods have opened an additional avenue to address these challenges. Ortiz et al.\cite{Kirchdoerfer2016Data-drivenMechanics} proposed a model-free computational framework where the specific form of a constitutive law is no longer needed, rather the stress fields are calculated by minimizing the distance between the state-space of the solution to the reference data space. This framework have been extended to computational elasticity \cite{Conti2018Data-DrivenElasticity}, in-elasticity \cite{Eggersmann2019Model-FreeInelasticity} as well as fracture mechanics~\cite{Carrara2020Data-drivenMechanics}. The model-free approach, albeit elegant, require huge amount of data and computational(optimization) time to ensure its fidelity, hence utilization of such approaches for history-dependent materials and complex geometries is prohibitive. On the other hand, several work have explored the possibility to apply deep neural network (NN) to approximate the constitutive relation of the materials. Mozaffar et al. \cite{Mozaffar2019DeepPlasticity} applied the recurrent neural network to study the Von-Mises plasticity and shown that the path dependency can be captured by the trained architecture.    

While most deep neural-network based approaches focused on the application of the developed tools from the machine learning community, which mainly designed for image processing (classification) and neural language processing (NLP) tasks. The 

\begin{figure}[!ht]
    \centering
    \includegraphics[height=8.5cm]{Figures/FE2Concept.PNG}
    \caption{graph representation of a multi-scale system.}
    \label{fig:multi-scale [representation}
\end{figure} 


==> old/macros.tex <==
\newcommand{\real}{\mathbb{R}}
\newcommand{\rE}{\mathbb{E}}
\newcommand{\rP}{\mathbb{P}}
\newcommand{\L}{\mathcal{L}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bF}{\boldsymbol{F}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\s}{\boldsymbol{s}}
\newcommand{\m}{\boldsymbol{m}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\Q}{\boldsymbol{Q}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\ep}{\epsilon}
\newcommand{\dep}{\dot{\epsilon}}
\newcommand{\bep}{\boldsymbol{\epsilon}}
\newcommand{\dbep}{\boldsymbol{\dot{\epsilon}}}
\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\ga}{\gamma}
\newcommand{\bga}{\boldsymbol{\gamma}}
\newcommand{\dga}{\dot{\gamma}}
\newcommand{\blm}{\boldsymbol{\lambda}}
\newcommand{\dblm}{\boldsymbol{\dot{\lambda}}}
\newcommand{\lm}{\lambda}
\newcommand{\dlm}{\dot{\lambda}}
\newcommand{\md}{\boldsymbol{\sigma}_{M}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\siginf}{{\sigma}_{\alpha}^{\infty}}
\newcommand{\bsig}{\boldsymbol{\sigma}}
\newcommand{\strain}{\varepsilon} 











